Exploring Challenges in Developing Edge-Cloud-Native Applications Across Multiple Business Domains

As the convergence of cloud computing and advanced networking continues to reshape modern software development, edge-cloud-native paradigms have become essential for enabling scalable, resilient, and agile digital services that depend on high-performance, low-latency, and reliable communication. This study investigates the practical challenges of developing, deploying, and maintaining edge-cloud-native applications through in-depth interviews with professionals from diverse domains, including IT, finance, healthcare, education, and industry. Despite significant advancements in cloud technologies, practitioners, particularly those from non-technical backgrounds-continue to encounter substantial complexity stemming from fragmented toolchains, steep learning curves, and operational overhead of managing distributed networking and computing, ensuring consistent performance across hybrid environments, and navigating steep learning curves at the cloud-network boundary. Across sectors, participants consistently prioritized productivity, Quality of Service, and usability over conventional concerns such as cost or migration. These findings highlight the need for operationally simplified, SLA-aware, and developer-friendly platforms that streamline the full application lifecycle. This study contributes a practice-informed perspective to support the alignment of edge-cloud-native systems with the realities and needs of modern enterprises, offering critical insights for the advancement of seamless cloud-network convergence.

==> src/background.tex <==

\begin{comment}

\section{Background}
\label{sec:background}

\hai{Don't know what are the technical contributions of this section to the paper. It appears to me that the section just provides text around cloud and FaaS which are already mentioned in the introduction.}

This section outlines the evolution from Industry 4.0 to Industry 5.0 and highlights how edge-cloud computing has emerged as a foundational enabler for these shifts. We also discuss challenges in developing edge-cloud-native applications, particularly within Function-as-a-Service (FaaS) systems.

% \subsection{Landscape of industrial framework and other domains}

% \textcolor{blue}{Historical background in real-world}

Historically, industrial transformations have focused on enhancing resource efficiency, increasing demand individualization, and reducing production cycles for cost effectiveness \cite{men2023research, ustundag2018conceptual}. These shifts have been encapsulated by conceptual frameworks that mirror prevailing technological and societal trends. Industry 4.0, for instance, emphasizes automation, interconnectivity, and real-time data exchange in cyber-physical systems \cite{enyoghasi2021industry, hassan2024systematic}. It has improved productivity, sustainability, and operational efficiency \cite{ghobakhloo2024industry, enyoghasi2021industry}. Building upon these foundations, Industry 5.0 introduces a human-centric perspective by promoting collaboration between humans and machines, with a strong emphasis on sustainability and resilience \cite{leng2022industry, alves2023industry, hassan2024systematic}. 


% \textcolor{red}{TODO: Clarify this sentence}

% This shift underscores the need for computing systems that not only balance autonomy with adaptability and technical power with contextual awareness, but also support both stable, machine-centric environments and resilient, human-centric paradigms capable of operating in highly dynamic conditions \cite{}.

% \subsection{Edge-Cloud-Native Applications Development Cycle}

\textcolor{red}{TODO: Repetitive information. Needs to be revised }
As the manufacturing sector transitions from cyber-physical systems to human-centric frameworks, similar movements are also emerging in domains such as healthcare, education, transportation, smart cities, and IoT systems. These changes are fueled by the need for adaptive, decentralized computing along with human-centric design requiring the capability of dynamic interactions with people \cite{}.


% \textcolor{blue}{Overview of the enabling technology--Serverless and Edge}

To meet the growing computational demands of modern environments—characterized by autonomy, dynamism, real-time responsiveness, and resilience—Serverless or Function-as-a-Service (FaaS) platforms have emerged as a critical enabler along with edge computing for edge-cloud-native application development \cite{tusa2024microservices}. By leveraging microservices architecture, automatic scaling, and infrastructure abstraction, FaaS simplifies the complexities of deploying and managing applications across heterogeneous and distributed edge-cloud environments \cite{deng2024cloud}. 


While the integration of serverless computing and edge technologies has successfully introduced lightweight, container-based infrastructures, it has also brought new complexities to cloud-native software development—particularly in ensuring service reliability and streamlining developer workflows. Due to the highly decoupled and modular nature of Function-as-a-Service (FaaS) systems, developers are often required to manually manage orchestration to ensure that applications exhibit the intended behavior \cite{}. However, since FaaS is inherently designed to support stateless functions that lack native data persistence between executions, coordinating stateful workflows and managing inter-function communication becomes a significant challenge \cite{}. 

Several studies \cite{} have aimed to alleviate the challenges of workflow management and stateful function development within FaaS-based architectures to streamline cloud-native application development. Although these efforts have introduced promising conceptual models and architectural patterns, their relevance often remains confined to theoretical domains. Many lack empirical validation in industrial environments and fall short of addressing key practical concerns such as scalability, developer experience, integration complexity, and cost-efficiency. This ongoing disconnect underscores the growing need to bridge the gap between academic research and real-world implementation challenges.

\end{comment}




